Progress on the QCD deconfinement critical point for $N_\text{f}=2$ staggered fermions

The global center symmetry of quenched QCD at zero baryonic chemical potential is broken spontaneously at a critical temperature $T_c$ leading to a first-order phase transition. Including heavy dynamical quarks breaks the center symmetry explicitly and weakens the first-order phase transition for decreasing quark masses until it turns into a smooth crossover at a $Z(2)$-critical point. We investigate the $Z(2)$-critical quark mass value towards the continuum limit for $N_\text{f}=2$ flavors using lattice QCD in the staggered formulation. As part of a continued study, we present results from Monte-Carlo simulations on $N_\tau=8,10$ lattices. Several aspect ratios and quark mass values were simulated in order to obtain the critical mass from a fit of the Polyakov loop to a kurtosis finite size scaling formula. Moreover, the possibility to develop a Ginzburg-Landau effective theory around the $Z(2)$-critical point is explored.

==> tikz/columbia-plot.tex <==
\begin{tikzpicture}[scale=0.44]
\def\a{10}
\def\b{10}
\def\centerarc[#1](#2)(#3:#4:#5)% Syntax: [draw options] (center) (initial angle:final angle:radius)
    { \draw[#1] ($(#2)+({#5*cos(#3)},{#5*sin(#3)})$) arc (#3:#4:#5 and #5*1.2 ); }
\coordinate (LB) at (0,0);
\coordinate (CB) at (\a/2,0);
\coordinate (RB) at (\a,0);
\coordinate (RC) at (\a,\b/2);
\coordinate (RT) at (\a,\b);
\coordinate (CT) at (\a/2,\b);
\coordinate (LT) at (0,\b);
\coordinate (LC) at (0,\b/2);
\coordinate (chiralB) at (\a/12*5,0);
\coordinate (chiralT) at (\a/32,\b);
\coordinate (PP) at (\a/5,\b/3*2);

\draw (LB) -- (RB) -- (RT) -- (LT) -- cycle;
\draw[gray] (LB) -- node[label={[rotate=45, color=black] below:\footnotesize{$\nf=3$}}]{} (RT);
\centerarc[blue,very thick, name path=C](RT)(180:270:\a*0.3);
\path[name path=BB](RB) -- (LB) -- (LT);
\path[name path=A] (chiralT) -- (LT) -- (LB) -- (chiralB);
\path[name path=D] (3/4*\a, \a) -- (RT) -- (\a, \a/4*3);
\tikzfillbetween[of=C and BB]{blue, opacity=0.1};
\tikzfillbetween[of=C and D]{yellow, opacity=0.2};
\draw[magenta,very thick, name path=B] (LT) -- (LB);
\node[anchor=north west, color=magenta] at (0,\b/8*7) {\footnotesize{$O(4)$}};



\node[anchor=north east] at (LB) {$0$};
\node[anchor=south west] at (RT) {$\infty$};
\node[anchor=north east] at (LT) {$m_s$};
\node[anchor=north east] at (RB) {$m_{u,d}$};
\node[anchor=south] at (CT) {\footnotesize{$\nf=2$}};
\node[anchor=north, rotate=90] at (RC) {\footnotesize{$\nf=1$}};
\fill[black] (PP) circle (\a/100);
\node[anchor=west] at (PP) {\footnotesize Physical Point};
\node[anchor=north] at (\a/3*2, \b/4) {\footnotesize\textit{Crossover}};
\node[anchor=north east, color=blue] at (\a/48*36,\b/24*21) {\footnotesize $Z(2)$};
\node[anchor=south east] at (\a*129/128,\b/16*14) {\footnotesize\textit{1. Order}};

\end{tikzpicture}
